Fooling Gaussian PTFs via Local Hyperconcentration

We give a pseudorandom generator that fools degree-$d$ polynomial threshold functions over $n$-dimensional Gaussian space with seed length $\mathrm{poly}(d)\cdot \log n$. All previous generators had a seed length with at least a $2^d$ dependence on $d$. The key new ingredient is a Local Hyperconcentration Theorem, which shows that every degree-$d$ Gaussian polynomial is hyperconcentrated almost everywhere at scale $d^{-O(1)}$.

==> finite-entropy.tex <==
%!TEX root = the-good-life3.tex


\section{The finite entropy argument:  Proof of \Cref{thm:main} using \Cref{thm:1}}
\label{sec:finite-entropy}

As discussed in the Introduction, we need to approximate an $n$-dimensional $\wise$-wise independent Gaussian $\by$ with a randomness-efficient $n$-dimensional random variable (call it $\bz$) to sufficiently high accuracy so that the scaled sum of $\len$ many independent copies of $\bz$, namely $\bigZ := \sqrt{\noisefixed}\bz_1 + \sqrt{\noisefixed} \bz_2 + \cdots + \sqrt{\noisefixed} \bz_{\len},$ is a random variable that $O(\epsprg)$-fools degree-$d$ PTFs. A similar task arose in \cite{kane11focs} and we use the machinery developed there to accomplish this task. In particular, we use the following two technical results from \cite{kane11focs}.

The first result states that it suffices to construct an $n$-dimensional random variable $\bz$ that can be coupled with a $\wise$-wise independent Gaussian $\by$ in such a way that for each coordinate $j \in [n]$, the values of $\bz_j$ and $\by_j$ are with high probability very close. This is the following:

\begin{lemma} [Lemma~21 of \cite{kane11focs}, adapted to our context] \label{lem:close-coords-fool}
Let $\bz$ be an $n$-dimensional random variable with the following property:  there is a coupling of $\bz$ with an $n$-dimensional $\wise$-wise independent Gaussian $\by$ which is such that for all $j \in [n]$ we have $\Pr[|\by_j - \bz_j| \geq \delta] \leq \delta$.  For $\len$ as specified at the start of \Cref{sec:high-level}, let $\bz_1,\dots,\bz_\len$ be independent random variables each distributed as $\bz$. Then the random variable $\bigZ := \sqrt{\noisefixed} \bz_1 + \cdots + \sqrt{\noisefixed} \bz_\len$
is an $\epsprg'$-PRG for degree-$d$ PTFs over Gaussian space, where $\epsprg' :=\parens*{\epsprg + O(n \len \delta + \degree \sqrt{n \len} \log(1/\delta) \delta^{1/\degree})}.$
\end{lemma}

The proof of \Cref{lem:close-coords-fool} is identical to the proof of Lemma~21 of \cite{kane11focs}, using \Cref{thm:1} rather than the analogous result from \cite{kane11focs} at the obvious point in the proof.

The second result states that an $n$-dimensional random variable $\bz$ as described above can indeed be generated in a randomness-efficient way:

\begin{lemma} [Implicit in the proof of Corollary~2 of \cite{kane11focs}]
There is an $n$-dimensional random variable $\bz$, that can be coupled with an $n$-dimensional $\wise$-wise independent Gaussian as described in \Cref{lem:close-coords-fool}, that can be generated with seed length $O(\wise \log(n/\delta)).$ 
\end{lemma}

\Cref{thm:main} follows from these two results by taking $\delta = (\epsprg)^{3 \degree} (\degree n \len)^{-3 \degree},$ since this choice leads to $\epsprg' = O(\epsprg)$ (see the proof of Corollary~2 of \cite{kane11focs} for the routine verification) and an overall seed length of
\[
O(\wise \len \log(n/\delta)) = \parens*{{\frac d \epsprg}}^{O(\log d)} \cdot \log n. \qed
\]


%\gray{Delete this eventually --- just towards making sure we end up with the right ultimate expression for \red{$fill-in$} for the seed length in the statement of \Cref{thm:main}: the seed length that pops out of this is
%\begin{align*}
%O(\wise \len \log(1/\delta)) &= O\parens*{\wise \len \parens*{\degree \log(1/\epsprg) + \degree\cdot (\log \degree + \log n + \log \len)}},
%\end{align*}
%right?}



==> hybrid-step-safe.tex <==
%!TEX root = the-good-life3.tex

\section{Proof of \Cref{thm:hybridstep}: one hybrid step} \label{sec:hybridstep}

In this section we define a collection of ``analysis checks,'' which are inequalities among the statistics, and explain the high-level structure of the proof of \Cref{thm:hybridstep}. The analysis checks  play a crucial role in the proof of \Cref{thm:hybridstep}: as we explain in \Cref{sec:high-level-one-step}, two very different arguments (corresponding to \Cref{lem:page14} and \Cref{lem:page13}) are used to establish the conclusion of \Cref{thm:hybridstep} at a given $x \in \R^n$, depending on whether or not all of the analysis checks hold at that $x$.


\subsection{Analysis checks} \label{sec:analysischecks}

In this subsection we define our set of ``analysis checks,'' which we denote $\AnalysisChecks$.  They are related to, but somewhat different from, the mollifier checks $\MollifierChecks$ that were used to define the mollifier $\allsoftchecks$ in \Cref{sec:defining-allsoftchecks}.

One difference between the analysis checks and the mollifier checks is that since the mollifier checks needed to be ``actually encoded into the mollifier,'' each one needed to consist of both an inequality $\ineq$ among the statistics and a ``softness'' parameter $\delta$.  In contrast, the analysis checks only play a role in our analysis and do not need to be encoded in the mollifier, and for this reason each analysis check consists only of an inequality $\ineq$ among the statistics.  Other than this, the difference between the analysis checks and mollifier checks is that the analysis checks essentially correspond to the mollifier checks ``shifted right by one in the grid.''

Below we describe the analysis checks in more detail and highlight the difference between them and the mollifier checks.



\begin{definition}
    The set $\AnalysisChecks$ contains the following checks (inequalities among statistics):\rasnote{Deliberately giving them ``positional names'' --- horizontal and diagonal checks --- here, as opposed to the ``semantic'' names for the mollifier checks (``noise insensitivity checks'' for the horizontal checks there, and ``strong anticoncentration checks'' for the diagonal checks there).  I'm hoping this difference in naming will make things clearer (less risk of it being confusing whether we are talking about a mollifier check or an analysis check).  If we end up disagreeing with this hope we can go to uniform terminology, but let's be conscious of what we do either way.}
    \begin{itemize}
        \item \textbf{The horizontal checks:} for every $0 \leq i \leq  d$, for every $1 \leq j \leq \maxcol-1$, we check that\rodnote{the parameter $\horzanal$ should probably be like $1/\maxcol$ in the below might not be exactly ideal}
            \begin{equation}    \label{eqn:horz-checks}
                \st_{i,j}(x) \approx_{\horzanal} \st_{i,j+1}(x)
                %\st_{i,1}(x) \in \left[ (1 - \horizclose) \st_{i,j}(x), (1 + \horizclose) \st_{i,j}(x)\right]
            \end{equation}
(so $2(\degree+1)(\maxcol-1)$ inequalities in total for the horizontal checks).
    \[
        \blue{\text{Let's take } \horzanal = \frac{1}{100d\maxcol}.}
    \]
  \rodnote{The following text may be inaccurate, as I changed the horz checks.}          Note that while the mollifier checks defined in \Cref{sec:MollifierChecks-def} check $\st_{i,0}(x)$ against $\st_{i,j}(x)$ for $j=0,\dots,\maxcol-1$, here we are checking $\st_{i,1}(x)$ against $\st_{i,j}(x)$ for $j=1,\dots,\maxcol$.  Thus these checks correspond precisely to the mollifier's noise-insensitivity checks, but ``shifted to the right by one.''
%            \emph{Please note:}  For reasons I don't 100\% understand yet, we \emph{don't} include the check $\ul{s}_{i,0} \approxeq \ul{s}_{i,1}$.  Instead, we use the \emph{Magic Lemma} (see below) to deal with $\ul{s}_{i,0}$.
        \item \textbf{The diagonal checks:} for \emph{just} the $1$st column (note, \emph{not} the $0$th column), for all $i=0,\dots,d-1,$ we check that\rodnote{is the 100 right?}
\begin{equation} \label{eqn:diag-checks}
                \blue{\st_{i+1,1}(x) \leq 100 \anticoncgap \st_{i,2}(x)}
\end{equation}
(so $d$ diagonal checks in total).
Note that while the strong anticoncentration checks defined in \Cref{sec:MollifierChecks-def} check $\st_{i+1,0}(x)$ against $\st_{i,1}(x)$, here we are checking $\st_{i+1,1}$ against $\st_{i,2}(x).$ So similar to the previous bullet, these checks correspond precisely to the mollifier's strong anticoncentration checks, but again ``shifted to the right by one.''

    \end{itemize}

    Below we give an illustration of the mollifier checks and of the analysis checks. \blue{Add suitable figure --- should replace what's below with a picture with diagonal checks}
    \myfig{.75}{diag2.png}{Analysis Checks}{}
\end{definition}



\subsection{High-level structure of the proof of \Cref{thm:hybridstep}} \label{sec:high-level-one-step}

%\gray{(Let's give some high level overview of the proof here --- some exposition, and state precisely \Cref{lem:page14,lem:page13}, and give a proof of \Cref{thm:hybridstep} using \Cref{lem:page14,lem:page13}.
%
%Some scavenged scraps below, slightly rephrased)}
%
%\bigskip
%
%[[[Get across that for the purpose of proving \Cref{thm:hybridstep}, we will introduce some ``Analysis Checks'' which are related to but somewhat different from the ``mollifier checks'' that go into defining $\allsoftchecks$. Forward reference to \Cref{sec:analysischecks}.]]]
%
%\bigskip

%\dots Now we go back to imagining $\bx = \ul{x}$ is fixed.  Given this $\ul{x}$, we will consider $\AnalysisChecks(\ul{\calS})$; i.e., all the analysis checks applied to the statistics $s_{i,j}(x)$.  We'll then prove the following two lemmas\rasnote{their union is Kane's Page 13 lemma, I think it's conceptually / expositionally cleaner to break them into two statements though}

Let us define the following small integer parameter,
\[
    \taylor = 4
\]
which will be the degree out to which we use Taylor's theorem.

\Cref{thm:hybridstep} will then be an immediate consequence of the below two lemmas, since
\[
    \blue{\textbf{gotta link up $\anticoncgap$ and $\epsprg/(8\len) = \noisefixed \epsprg/8$}}.
\]
\begin{lemma} [If analysis checks pass, $\wise$-wise moments determine mollifier's value] \label{lem:page14}
Suppose that $x \in \R^n$ is such that all of the checks in $\AnalysisChecks$ hold at $x$, and that the random vector $\by$ is a $\wise$-wise independent  $n$-dimensional Gaussian.  Then $\E\bracks*{\Indplus\parens*{\sqrt{1-\noisefixed} \cdot x + \sqrt{\noisefixed}\cdot \by}}$ is determined up to an additive $\pm \poly(d^\taylor) \cdot \anticoncgap^{\taylor/2}$.\rodnote{this bound may not be quite right; also the $\poly()$ also hides some factors like $\taylor^\taylor$; gotta find a way to say this briefly}
\end{lemma}

\begin{lemma} [If an analysis check fails, mollifier is close to zero] \label{lem:page13}
Suppose that $x \in \R^n$ is such that some check in $\AnalysisChecks$ does not hold at $x$, and that the random vector $\by$ is a $\wise$-wise independent  $n$-dimensional Gaussian.  Then $\E\bracks*{\Indplus\parens*{\sqrt{1-\noisefixed} \cdot x + \sqrt{\noisefixed}\cdot \by}} \in [0,\poly(d^\taylor) \cdot \anticoncgap^{\taylor/2}]$.
\end{lemma}

As we will see in the following sections, two very different arguments are used to prove \Cref{lem:page14} and \Cref{lem:page13}. \Cref{lem:page14}, which corresponds to the case in which $x$ is such that all of the analysis checks pass, is based on a Taylor's theorem argument.  In contrast, \Cref{lem:page13}, which corresponds to the case in which $x$ is such that some analysis check fails, employs a delicate argument, which takes advantage of the careful way that the analysis checks are structured vis-a-vis the mollifier checks, to argue that  in this case almost all outcomes of $\by$ result in $\Indplus\parens*{\sqrt{1-\noisefixed} \cdot x + \sqrt{\noisefixed}\cdot \by}=0$.

Before we can enter into the proofs of \Cref{lem:page14} and \Cref{lem:page13}, there are several intermediate technical results which will be used in both proofs which we need to establish.  \rasnote{This might be a good place to eventually stick in some exposition about what these technical results --- Desideratum \#2, Magic Lemma ---  are, and why they arise in both of the \Cref{lem:page14} and \Cref{lem:page13} proofs.} We state and prove these technical results in  \Cref{sec:hypervariance-bound} and \Cref{sec:magic-lemma}, and prove \Cref{lem:page14} and \Cref{lem:page13} in \Cref{sec:page14} and \Cref{sec:page13} respectively.




==> kane-original.tex <==
\section{Appendix by Daniel Kane}    \label{app:kane}

\newcommand{\var}{\mathbf{Var}}
\newcommand{\cov}{\mathbf{Cov}}
%\newcommand{\eps}{\epsilon}
\renewcommand{\R}{\mathbb{R}}
\newcommand{\pr}{\mathbf{Pr}}
%\newcommand{\poly}{\mathrm{poly}}
\renewcommand{\E}{\mathbb{E}}
\newcommand{\hypvar}{\mathrm{HyperVar}}
\newcommand{\D}{\mathcal{D}}


\begin{lemma}\label{anticoncentration lemma}
Let $p$ be a degree-$d$ polynomial with $p(x)\geq 0$ for all $x$. Then if $X$ is a random Gaussian and $\eps > 0$ we have that
$$
\pr(p(X) < \eps \E_X[p(X)]) = O(d \eps^{1/d}).
$$
\end{lemma}
\begin{proof}
This follows from Carbery-Wright and the observation that $|p(X)|_2 \geq \E[p(X)]$.
\end{proof}

\begin{theorem}\label{main theorem}
There exists a constant $c>0$ so that for any $1>\eps,\beta>0$ and $R\geq 1$ sufficiently small if $(g_\nu)$ is a nice distribution over degree-$d$ polynomials in $n$ variables then for
$$
\lambda \leq \frac{c\eps \beta}{R d^{9/2}}
$$
then for $x\sim G^n$ with probability at least $1-\beta$ we have that
$$
\E_\nu[\hypvar_R((g_\nu)_{\lambda|x})] \leq \eps^2 \E_\nu [ \| (g_\nu)_{\lambda|x}\|_2^2 ].
$$
\end{theorem}
\begin{proof}
The proof of this theorem will depend on basic facts about the sequence of derivatives of $(g_\nu)_{\lambda|x}$. Firstly, we establish some notation, we let $D_Y f(X)$ denote the directional derivative of $f$ at $X$ in the $Y$ direction. We begin with the following Lemma relating the size of functions and their derivatives:
\begin{lemma}\label{strong anticoncentration lemma}
Let $(g_\nu)$ be a nice distribution over degree-$d$ polynomials. Let $X$ and $Y$ be independent Gaussian random variables. Then for $\eps>0$ we have that
$$
\pr_{X,Y}(\E_\nu [|g_\nu(X)|^2] \leq \eps^2 \E_\nu [|D_Y (g_\nu(X))|^2]) = O(d^2\eps).
$$
\end{lemma}
\begin{proof}
We begin with the case where $g_\nu$ is actually a constant family (i.e. is just a single function). This result then follows immediately from Lemma 9 of [D. Kane ``The Correct Exponent for the Gotsman-Linial Conjecture''].

From here we generalize to the case where $g_\nu$ is a linear polynomial in $\nu$. by the previous case, we have that
$$
\pr_{X,Y,\nu}(|g_\nu(X)|^2 \leq \eps^2 |D_Y (g_\nu(X))|^2) = O(d^2\eps).
$$
On the other hand since $g_\nu(X)$ and $D_Y (g_\nu(X))$ are linear functions of $\nu$. Therefore, for any $X$ and $Y$, with at least $50\%$ probability over the choice of $\nu$ we have that $\E_\nu[|g_\nu(X)|^2 ] \ll |g_\nu(X)|^2$ and $|D_Y (g_\nu(X))|^2 \ll \E_\nu[|D_Y (g_\nu(X))|^2]$. Therefore, whenever
$$
\E_\nu [|g_\nu(X)|^2] \leq \eps^2 \E_\nu [|D_Y (g_\nu(X))|^2]
$$
there is at least a $50\%$ probability over the choice of $\nu$ that
$$
|g_\nu(X)|^2 \leq \eps^2 C |D_Y (g_\nu(X))|^2
$$
for some positive constant $C$. However, the latter happens with probability $O(d^2 \eps)$ and is at least half of
$$
\pr_{X,Y}(\E_\nu [|g_\nu(X)|^2] \leq \eps^2 \E_\nu [|D_Y (g_\nu(X))|^2]).
$$
Therefore, this latter probability is $O(d\eps^2).$

Finally, we can handle the generic case. Let $h_a(\nu)$ be an orthonormal basis for the polynomials in $\nu$. We can write $g_\nu(x)$ as $\sum_a h_a(\nu)p_a(x)$ for some polynomials $p_a$. Define
$$
h_\mu(x):= \sum_a \mu_a p_a(x)
$$
where $\mu$ is a Gaussian random variable with as many components as there are terms in the above decomposition of $g_\nu$. It is easy to see that for any $X$ and $Y$ that
$$
\E_\nu[|g_\nu(X)|^2] = \sum_a p_a^2(X) = \E_\mu[|h_\mu(X)|^2]
$$
and
$$
\E_\nu[|D_Y g_\nu(X)|^2] = \sum_a (D_Y p_a(X))^2 = \E_\mu[|D_Y h_\mu(X)|^2].
$$
Since our Lemma holds for $h$, it must therefore also hold for $g$. This completes our proof.
\end{proof}

Our theorem will rest upon the following notion of a random derivative sequence:
\begin{definition}
Given a nice distribution $(g_\nu)$ of degree-$d$ polynomials, a \emph{random derivative sequence} for $g$ is a sequence of the form
$$
\E_\nu[|g_\nu(X)|^2], \E_\nu[|D_{Y_1}g_\nu(X)|^2], \E_\nu[|D_{Y_2}D_{Y_1}g_\nu(X)|^2], \ldots \E_\nu[|D_{Y_d}D_{Y_{d-1}}\cdots D_{Y_1}g_\nu(X)|^2],
$$
where $X,Y_1,Y_2,\ldots,Y_d$ are independent Gaussian random variables.

We will often denote the $k^{th}$ term by
$$
\D^k_{X,Y_i}(g_\nu) :=\E_\nu[|D_{Y_k}D_{Y_{k-1}}\cdots D_{Y_1}g_\nu(X)|^2].
$$
\end{definition}

\begin{corollary}\label{derivative sequence corollary}
Let $(g_\nu)$ be a nice distribution over degree-$d$ polynomials. Then with probability at least $1-\eps$ over the choice of $X,Y_i$ we have that:
$$
\D^{k+1}_{X,Y_i}(g_\nu) = O(d^6/\eps^2)\D^{k}_{X,Y_i}(g_\nu)
$$
for all $0\leq k \leq d$.
\end{corollary}
\begin{proof}
It follows immediately from Lemma \ref{strong anticoncentration lemma} that for each $k$
$$
\D^{k+1}_{X,Y_i}(g_\nu) = O(d^6/\eps^2)\D^{k}_{X,Y_i}(g_\nu)
$$
with probability $1-\eps/d$. The full result follows from a union bound over $k$.
\end{proof}

This says that a typical random derivative sequence does not increase too rapidly. However, we show that there is a kind of converse for non-hyperconcentrated families:
\begin{proposition}\label{sequence increase proposition}
Let $(g_\nu)$ be a nice distribution of degree-$d$ polynomials so that for some $R,\eps>0$ we have that
$$
\E_\nu[\hypvar_R((g_\nu))] \geq \eps^2 \E_\nu [ \| (g_\nu)\|_2^2 ].
$$
Then with at least $50\%$ probability over a choice of random Gaussians $X,Y_i$ we have that for some $0\leq k \leq d$ that
$$
\D^{k+1}_{X,Y_i}(g_\nu) > \Omega(\eps^2/(d^3 R^2))\D^{k}_{X,Y_i}(g_\nu).
$$
\end{proposition}

In order to prove this, we will need to talk about the Hermite parts of $g$.
\begin{definition}
Let $g$ be a polynomial. Then $g^{[k]}$ denotes the degree-$k$ Hermite part of $g$.
\end{definition}

We will make use of the following facts:
\begin{fact}
For any polynomial $g$ and $R>0$,
$$
\hypvar_R(g) = \sum_k k R^{2k} \|g^{[k]}\|_2^2.
$$
\end{fact}
\begin{fact}
For any polynomial $g$ and vector $v$:
$$
(D_v g)^{[k]} = D_v(g^{[k+1]}).
$$
\end{fact}
\begin{fact}
For any $g$ with $g=g^{[k]}$ and $X$ a random Gaussian
$$
\E_X [\| D_X g \|_2^2] = k\|g\|_2^2.
$$
\end{fact}

We will also need to know that with reasonable probability that some element of a random derivative sequence is not too small.
\begin{lemma}\label{decrease lemma}
Let $(g_\nu)$ be a nice distribution of degree-$d$ polynomials and let $m\geq d$. Then with probability at least $1-d/m$ over a choice of random Gaussians $X,Y_i$ there exists a $0\leq k\leq d$ so that
$$
\D^{k}_{X,Y_i}(g_\nu) \geq \Omega(1/m)^{3k} \E_\nu[ \|g_\nu\|_2^2]/2.
$$
\end{lemma}
\begin{proof}
We proceed by induction on $d$. If $d=0$, then $\D^{0}_{X,Y_i}(g_\nu) = \E_\nu[ \|g_\nu\|_2^2]$ and we are done.

For the inductive step, we break into two cases. On the one hand, if
$$
\E_\nu[ \|g_\nu\|_2^2] \geq 100m \E_\nu[\var_X(g_\nu(X))],
$$
then we have that
\begin{align*}
& \E_X[\E_{\nu}[\|g_\nu\|_2^2 \mathbf{1}\{|g_\nu(X)| < (2/3)\|g_\nu\|_2\}]]\\
= &\E_\nu[\E_X[\|g_\nu\|_2^2 \mathbf{1} \{|g_\nu(X)| < (2/3)\|g_\nu\|_2\}]]\\
\leq & \E_\nu\left[9(\|g_\nu\|_2^2)\left(\frac{\var_X(g_\nu(X))}{\|g_\nu\|_2^2} \right)\right]\\
= & 9\E_\nu[ \|g_\nu\|_2^2]/2\\
\leq & (1/10m) \E_\nu[ \|g_\nu\|_2^2].
\end{align*}
However, if
$$
\D^{0}_{X,Y_i}(g_\nu) < \E_\nu[ \|g_\nu\|_2^2]/2,
$$
it must be the case that
$$
\E_{\nu}[\|g_\nu\|_2^2 \mathbb{1}\{|g_\nu(X)| < (2/3)\|g_\nu\|_2\}] \geq (1/6) \E_{\nu}[\|g_\nu\|_2^2],
$$
and by the Markov Inequality, this happens with probability at most $1/m$.

On the other hand, if
$$
\E_\nu[ \|g_\nu\|_2^2] \leq 100m \E_\nu[\var_X(g_\nu(X))],
$$
then
$$
\E_{Y_1}[\E_\nu[\|D_{Y_1} g_\nu\|_2^2]] = \E_\nu[\var_X(g_\nu(X))].
$$
Since $\E_\nu[\|D_{Y_1} g_\nu\|_2^2]$ is a non-negative quadratic function of $Y_1$, Lemma \ref{anticoncentration lemma} implies that with probability at least $1-1/m$ we have that
$$
\E_\nu[\|D_{Y_1} g_\nu\|_2^2] \geq (1/m^2) \E_\nu[\var_X(g_\nu(X))] \geq \Omega(1/m^3)\E_\nu[ \|g_\nu\|_2^2].
$$
For such a $Y_1$, we can apply our inductive hypothesis to $(D_{Y_1}g_\nu)$.
\end{proof}

We are now prepared to prove Proposition \ref{sequence increase proposition}
\begin{proof}
Note that
$$
\E_\nu[\hypvar_R(g_\nu)] = \sum_{k=1}^d k R^{2k} \E_\nu[\|g_\nu^{[k]}\|_2^2].
$$
Therefore, under our hypothesis, there must be a $k$ so that
$$
\E_\nu[\|g_\nu^{[k]}\|_2^2] \geq (\eps^2/(4R^2))^k\E_\nu[\|g_\nu\|_2^2].
$$
Notice that
$$
\E_{\nu}[\| D_{Y_k}D_{Y_{k-1}}\cdots D_{Y_1}g_\nu^{[0]}\|_2^2]
$$
is a non-negative degree $2k$ polynomial in $Y_1,\ldots,Y_k$ with average value at least $(\eps^2/(4R^2))^k\E_\nu[\|g_\nu\|_2^2]$. Therefore, Lemma \ref{anticoncentration lemma} implies that with probability at least $5/6$ we have that
$$
\| D_{Y_k}D_{Y_{k-1}}\cdots D_{Y_1}g_\nu^{[0]}\|_2^2 \geq \Omega(\eps^2/(d^2 R^2))^k \E_\nu[\|g_\nu\|_2^2].
$$
By Lemma \ref{decrease lemma} with probability at least $5/6$ there is a $k' > k$ so that
$$
\D^{k'}_{X,Y_i}(g_\nu) \geq \Omega(1/d)^{3(k'-k)}\| D_{Y_k}D_{Y_{k-1}}\cdots D_{Y_1}g_\nu^{[0]}\|_2^2/2 \geq \Omega(\eps^2/(d^3 R^2))^{k'}\E_\nu[\|g_\nu\|_2^2].
$$
Finally, with probability at least $5/6$ we have that
$$
\D^{0}_{X,Y_i}(g_\nu) = O(1)\E_\nu[\|g_\nu\|_2^2].
$$
Thus, if all three of these events hold (which happens with probability at least $1/2$), there will be some $d\geq k> 1$ so that
$$
\D^{k}_{X,Y_i}(g_\nu) \geq \Omega(\eps^2/(d^3 R^2))^{k}\D^{0}_{X,Y_i}(g_\nu).
$$
Therefore, there must also be a $k$ so that
$$
\D^{k+1}_{X,Y_i}(g_\nu)\geq \Omega(\eps^2/(d^3 R^2)) \D^{k}_{X,Y_i}(g_\nu).
$$
\end{proof}

Our Theorem will now follow from the tension between Corollary \ref{derivative sequence corollary} and Proposition \ref{sequence increase proposition} along with the observation that
$$
\D^k_{X,Y_i}((g_\nu)_{\lambda|x}) = \lambda^{2k} \D^k_{Z,Y_i}(g_\nu)
$$
where $Z=\sqrt{1-\lambda}x+\lambda X$. Note also that $Z$ is a standard Gaussian in $X$ and $x$ are. In particular, Corollary \ref{derivative sequence corollary} tells us that with probability $1-\beta/2$ that
\begin{equation}\label{derivative upper bound equation}
\D^{k+1}_{Z,Y_i}(g_\nu) = O(d^6/\beta^2)\D^k_{Z,Y_i}(g_\nu)
\end{equation}
for all $0\leq k \leq d$. On the other hand, if
$$
\E_\nu[\hypvar_R((g_\nu)_{\lambda|x})] > \eps^2 \E_\nu [ \| (g_\nu)_{\lambda|x}\|_2^2 ]
$$
then Proposition \ref{sequence increase proposition} implies that with at least $50\%$ probability that there is a $0\leq k\leq d$ so that
$$
\D^{k+1}_{X,Y_i}((g_\nu)_{\lambda|x}) > \Omega(\eps^2/(d^3 R^2))\D^{k}_{X,Y_i}((g_\nu)_{\lambda|x}).
$$
But this is equivalent to saying that
$$
\D^{k+1}_{Z,Y_i}(g_\nu) > \Omega(\lambda^{-2}\eps^2/(d^3 R^2))\D^k_{Z,Y_i}(g_\nu).
$$
However, given our setting of $\lambda$ this would contradict Equation \eqref{derivative upper bound equation}. Therefore, the probability of Equation \eqref{derivative upper bound equation} being violated is at most $\beta/2$, but is at least half the probability that
$$
\E_\nu[\hypvar_R((g_\nu)_{\lambda|x})] > \eps \E_\nu [ \| (g_\nu)_{\lambda|x}\|_2^2 ].
$$
Hence we conclude that the latter probability is at most $\beta.$
\end{proof}


==> lit-safe.tex <==
%!TEX root = the-good-life3.tex


\section{Proof of \Cref{lem:page13}:  if an analysis check fails, then whp a mollifier check fails (Lost in Translation / the Kane p. 13 argument)} \label{sec:page13}

As in the previous section,\rodnote{is this true?} we completely fix an $x = \ul{x} \in \R^n$. Suppose first that $\by \sim \normal(0,1)^n$, and let us introduce the notation
\[
    \ul{\st}_{i,j} = \st_{i,j}(\ul{x}), \qquad \bs_{i,j} = \st_{i,j}(\sqrt{1-\noisefixed} \ul{x} + \sqrt{\noisefixed} \by).
\]
We will use the following facts.  First, by definition we have that for all $0 \leq i \leq d$ and all $0 \leq j \leq \maxcol-1$,
\begin{equation} \label{eqn:themean}
    \ul{\st}_{i,j+1} = \E[\bs_{i,j}] = \abs{\E[\bs_{i,j}]}.
\end{equation}
\rodnote{I think we should actually put all these deductions right after \Cref{thm:desideratum2} appears, as corollaries}
Second, by \Cref{thm:desideratum2} we have that for all $0 \leq i \leq d-1$ and all $0 \leq j \leq \maxcol-1$,
\[
    \HV_{\frac{\sqrt{\hyperfixed}}{13}}[\bs_{i,j}]
    \leq 16 \max\{\ul{\st}_{i,j+1} \cdot \ul{\st}_{i+1,j}, \ul{\st}_{i+1,j}^2\}.
\]
%Now suppose we happen to know $\ul{\st}_{i+1,j} \leq \theta \ul{\st}_{i,j+1}$ for some $0 \leq \theta \leq 1$.  Then we would conclude
%\[
%    \HV_{\frac{\sqrt{\hyperfixed}}{13}}[\bs_{i,j}]  \leq 16 \theta \ul{\st}_{i,j+1}^2 = 16 \theta \E[\bs_{i,j}]^2.
%\]
Combining with \Cref{lem:hypervar-to-hypercon}, and using
\[
    \blue{1+\hyperfixed/13 \geq \taylor},
\]
we conclude:
\begin{equation}    \label[ineq]{ineq:useme}
    \text{for $0 \leq i \leq d-1$, $0 \leq j \leq \maxcol-1$,} \quad \bs_{i,j} \text{ is } (\taylor, 4\max\{\sqrt{\zeta_{i,j}}, \zeta_{i,j}\})\text{-hyperconcentrated,} \quad \zeta_{i,j} = \frac{\ul{\st}_{i+1,j}}{\ul{\st}_{i,j+1}}
\end{equation}
(where we interpret $0/0=0$). In this deduction, although $\bs_{i,j}$ was originally defined with $\by \sim \normal(0,1)^n$, the conclusion remains true if $\by$ merely satisfies \Cref{ass} with \blue{$k = 2\taylor d$}.\rodnote{I do not do a good job in this section of explaining why everything only depends on low-degree moments of~$\by$.}  We will henceforth only use \Cref{ineq:useme}, so it will be fine to proceed only assuming $\by$ satisfies \Cref{ass}.  Our goal now\rodnote{this is not organized well; re-organize properly later} is to show that, assuming $\ul{x}$ causes one of the analysis checks to fail, we have
\[
    0 \leq \E[\Indplus(\sqrt{1-\noisefixed} \cdot \ul{x} + \sqrt{\noisefixed} \cdot \by)] \leq \poly(d^\taylor) \cdot \anticoncgap^{\taylor/2}.
\]
Recall that $\Indplus$ is the product of functions bounded in $[0,1]$; namely, the indicator of $\sgn(p) = +1$, and all of the  $\softcheck_\chk$ functions, $\chk \in \MollifierChecks$.  Thus it will suffice to show, assuming $\ul{x}$ causes one of the analysis checks to fail, that:
\begin{multline}
    \text{There exists some } \chk \in \MollifierChecks \text{ ``$s_u \geq c s_v$ with softness~$\softness$''}, \\
     \text{such that } \softcheck_\chk(\sqrt{1-\noisefixed} \cdot \ul{x} + \sqrt{\noisefixed} \cdot \by) = 0 \text{ --- equivalently, } \bs_{u} \leq \exp(-\softness) \cdot c \bs_v \text{ ---} \\
         \text{except with probability at most } \poly(d^\taylor) \cdot \anticoncgap)^{\taylor/2}. \label[ineq]{ineq:muffin}
\end{multline}


To establish this, we will consider the checks in $\AnalysisChecks$ in a careful order; specifically, the order shown below
\blue{The following is not quite right --- needs to be replaced with a picture with diagonal checks, and made a bit more formal}
%\myfig{.75}{diag4.png}{Ordering of analysis Checks}{}

\myfig{.75}{lostInTrans.png}{Ordering of analysis Checks}{}

\bigskip

We split into cases depending on the first analysis check that fails for~$\ul{x}$.




\subsection{The first failing analysis check is horizontal in the bottom row ($i=d$)}
Recall that the analysis checks in the bottom row are $\ul{\st}_{d,j} \approx_{\horizanal} \ul{\st}_{d,j+1}$ for all $1 \leq j \leq \maxcol-1$.\rodnote{Is this correct?}  But \Cref{def:si0} and \Cref{fact:deriv-deg} imply that $\st_{d,0}$ is a \emph{constant} function, and it follows from \Cref{def:sij} that $\st_{d,j}$ is the \emph{same} constant function for all~$j$.  Thus all numbers $\ul{\st}_{d,j}$ are equal to the same constant, and hence the analysis checks in the bottom row cannot actually fail.  In other words, this case cannot occur.

\subsection{The first failing analysis check is horizontal, but not in the bottom row}
Suppose that the first failing analysis check is one of the two implicit in the statement
\begin{equation}    \label{eqn:horzfail}
    \ul{\st}_{i^*,j^*} \not \approx_{\horizanal} \ul{\st}_{i^*,j^*+1},
\end{equation}
for some $0 \leq i^* \leq d-1$ and $1 \leq j^* \leq \maxcol - 1$.  In this case we study the random variables $\bs_{i^*, j^*-1}$ and $\bs_{i^*, j^*}$. By \Cref{eqn:themean} we have
\begin{equation} \label{eqn:damean}
    \E[\bs_{i^*,j^*-1}] = \ul{\st}_{i^*,j^*}, \qquad \E[\bs_{i^*,j^*}] = \ul{\st}_{i^*,j^*+1}, \qquad \text{and let us write } M = \max\{ \ul{\st}_{i^*,j^*}, \ul{\st}_{i^*,j^*+1} \}.
\end{equation}
Since we are at the first failing analysis check, we know that all horizontal analysis checks in the $(i^*+1)$-th row passed:
\[
    \ul{\st}_{i^*+1,j} \approx_{\horizanal} \ul{\st}_{i^*+1,j+1} \quad \forall\ 1 \leq j \leq \maxcol-1,
\]
and hence
\[
    \ul{\st}_{i^*+1,j} \approx_{\maxcol \horizanal} \ul{\st}_{i^*+1,1} \quad \forall\ 1 \leq j \leq \maxcol,
\]
and hence by \Cref{lem:magicker-lemma} \red{make sure everything is really synched up and plumbed for the magic lemma} we can extend (a slightly weaker version of) this deduction even to the $j = 0$ case:
\[
    \ul{\st}_{i^*+1,j} \approx_{1} \ul{\st}_{i^*+1,1} \quad \forall\ 0 \leq j \leq \maxcol.
\]
As a further consequence of the fact that we are at the first failing analysis check, we know that the diagonal analysis check relating the $(i^*+1)$-th to the $i^*$-th row passed:
\[
    \ul{\st}_{i^*+1,1} \leq 100 \anticoncgap \ul{\st}_{i^*,2}.
\]
Putting these deductions about preceding passing checks together, we conclude
\[
    \ul{\st}_{i^*+1,j} \leq 100 e \anticoncgap \ul{\st}_{i^*,2} \quad \forall\ 0 \leq j \leq \maxcol.
\]
Also, by \Cref{ineq:useme},
\[
    \bs_{i^*,j^*-1} \text{ is } (\taylor, 4\max\{\sqrt{\zeta_{i^*,j^*-1}}, \zeta_{i^*,j^*-1}\})\text{-hyperconcentrated,} \quad \zeta_{i^*,j^*-1} = \frac{\ul{\st}_{i^*+1,j^*-1}}{\ul{\st}_{i^*,j^*}}
    \leq \frac{100e \anticoncgap \ul{\st}_{i^*,2}}{\ul{\st}_{i^*,j^*}},
\]
\[
    \bs_{i^*,j^*} \text{ is } (\taylor, 4\max\{\sqrt{\zeta_{i^*,j^*}}, \zeta_{i^*,j^*}\})\text{-hyperconcentrated,} \quad \zeta_{i^*,j^*} = \frac{\ul{\st}_{i^*+1,j^*}}{\ul{\st}_{i^*,j^*+1}} \leq \frac{100e \anticoncgap \ul{\st}_{i^*,2}}{\ul{\st}_{i^*,j^*+1}}.
\]
Regarding the $\ul{\st}_{i^*,2}$ in both numerators,   we consider two cases.  If $j^* = 1$, then $\ul{\st}_{i^*, 2} = \ul{\st}_{i^*, j^*+1} \leq M$.  Otherwise, by virtue of the fact that all preceding analysis checks in the $i^*$-th row passed, we conclude that $\ul{\st}_{i^*,2} \approx_{\maxcol \horizanal} \ul{\st}_{i^*,j^*}$ and hence $\ul{\st}_{i^*,2} \leq eM$ (as $\maxcol \horizanal \leq e$).  Either way, we conclude
\begin{equation} \label[ineq]{ineq:pumpkin}
    \zeta_{i^*,j^*-1}  \leq \frac{100e^2 \anticoncgap M}{\ul{\st}_{i^*,j^*}}, \quad \zeta_{i^*,j^*}  \leq \frac{100e^2 \anticoncgap M}{\ul{\st}_{i^*,j^*+1}}.
\end{equation}
From this point on, we will make the exact same deductions about $\bs_{i^*,j^*-1}$ and $\bs_{i^*,j^*}$.  Let us write $\bs$ to denote either, similarly write just $\zeta$, and write $\mu = \E[\bs]$ (recalling \Cref{eqn:damean}).   \Cref{ineq:pumpkin} tells us that $\zeta \leq 100 e^2 \anticoncgap M / \mu$.  Take $t = \frac{M/\mu}{d^{\blue{12345}}}$ and apply \Cref{prop:hypermarkov}\rodnote{We should give this a name, like ``hyper-Markov'' or something} to deduce that
\[
    |\bs - \mu| \leq M/d^{12345}  \text{ except with probability at most } \parens*{\frac{4\max\{\sqrt{\zeta},\zeta\}\cdot d^{12345}}{M/\mu}}^\taylor \leq \poly(d^\taylor) \cdot \anticoncgap^{\taylor/2}
\]
(using $M/\mu \geq 1$, $\anticoncgap \leq 1$). Thus except with the desired failure probability, each of $\bs_{i^*,j^*-1}, \bs_{i^*,j^*}$ is within $M/d^{12345}$ of its mean.  Without loss of generality, assume $\bs_{i^*,j^*}$ has the larger mean; thus \Cref{eqn:horzfail} tells us that
\[
    \ul{\st}_{i^*,j^*} \leq \exp(-\horizanal) \ul{\st}_{i^*,j^*+1} = \exp(-\horizanal) M.
\]
Now even in the ``worst case'' that $\ul{\st}_{i^*,j^*} = \exp(-\horizanal) M$, we still have that $\bs_{i^*,j^*-1}$ is within $M/d^{12345}$ of $\exp(-\horizanal) M$ and $\bs_{i^*,j^*}$ is within $M/d^{12345}$ of $M$, except with probability $\poly(d^\taylor) \cdot \anticoncgap^{\taylor/2}$.  This establishes \Cref{ineq:muffin} for the $(i^*,j^*-1)$~vs.~$(i^*,j^*)$\rodnote{Note that indeed this cannot be in the last possible column, which is good because the mollifier does not check this last column!} noise insensitivity mollifier check (\blue{using $1/d^{12345} \ll$ the ratio checked in the mollifier}).




\subsection{The first failing analysis check is diagonal}
Suppose that the first failing analysis check is
\[
    \ul{\st}_{i^*+1,1} \not \leq 100 \anticoncgap \ul{\st}_{i^*,2}
\]
for some $0 \leq i^* \leq d-1$.  In this case we study the random variables $\bs_{i^*+1, 0}$ and $\bs_{i^*, 1}$.  By \Cref{eqn:themean} and the above inequality we have
\begin{equation}    \label[ineq]{ineq:firstdiag}
    \E[\bs_{i^*+1,0}] = \ul{\st}_{i^*+1,1} > 100 \anticoncgap \ul{\st}_{i^*,2} = 100 \anticoncgap \E[\bs_{i^*,1}].
\end{equation}
\begin{claim}   \label{claim:imhungry}
    $\bs_{i^*+1,0} \geq \frac12 \ul{\st}_{i^*+1,1}$ except with probability at most $(80e)^{\taylor} \cdot \anticoncgap^{\taylor/2}$.
\end{claim}
\begin{proof}
    The claim is immediate from \Cref{prop:hypermarkov} once we establish the following:
    \begin{equation}    \label[ineq]{ineq:pizza}
        \bs_{i^*+1, 0} \text{ is } (\taylor, 40e\sqrt{\anticoncgap})\text{-hyperconcentrated.}
    \end{equation}
    To show \Cref{ineq:pizza}, first suppose $i^*+1 = d$.  Then $\st_{i^*+1,0}$ is a constant function, hence $\bs_{i^*+1,0}$ is a constant random variable, and \Cref{ineq:pizza} is clearly true.  Otherwise, we complete the proof assuming $i^*+1 < d$.  In this case we may conclude that there was at least one ``earlier'' diagonal analysis check, and it succeeded:
    \[
        \ul{\st}_{i^*+2,1} \leq 100 \anticoncgap \ul{\st}_{i^*+1,2}.
    \]
    Further, the horizontal analysis checks in ``rows'' $i^*+1$ and $i^*+2$ all succeeded, and hence
    \[
        \ul{\st}_{i^*+1,2} \approx_{\horizanal} \ul{\st}_{i^*+1,1}, \qquad \ul{\st}_{i^*+2,1} \approx_{1} \ul{\st}_{i^*+2,0}, 
    \]
    where to get the second approximate equality here we had to use \Cref{lem:magicker-lemma} \red{make sure everything is really synched up and plumbed for the magic lemma}.
    \blue{Upper-bounding $e^{\horizanal}$ by $e$ for simplicity}, we deduce
    \[
        \ul{\st}_{i^*+2,0} \leq 100 e^2 \anticoncgap \ul{\st}_{i^*+1,1}.
    \]
    Now \Cref{ineq:pizza} follows from \Cref{ineq:useme}.\rodnote{Surely we're not required to explicitly point out that $e^2 \anticoncgap \leq 1$.}
\end{proof}

\begin{claim}
    $\bs_{i^*,1} \leq  \ul{\st}_{i^*+1,1}/(20\anticoncgap)$ except with probability at most $(8/10)^\taylor \cdot \anticoncgap^{\taylor/2}$.
\end{claim}
\begin{proof}
    \rodnote{The following looks more complicated than it really is.  It's kind of only complicated-looking because I felt like using \Cref{ineq:useme} as a black box.  If you just use the ingredients that go into \Cref{ineq:useme} instead, it's more natural-looking\dots}By \Cref{ineq:useme}, $\bs_{i^*,1}$ is $(\taylor, 4\max\{\sqrt{\zeta_{i^*,1}},\zeta_{i^*,1}\})$-hyperconcentrated, and  \Cref{ineq:firstdiag} tells us that $\zeta_{i^*,1}/ \anticoncgap > 100$.  Taking $t = \zeta_{i^*,1}/(20\anticoncgap) - 1 > \zeta_{i^*,1}/(2\anticoncgap)$ in \Cref{prop:hypermarkov}, we conclude that
    \[
        \bs_{i^*,1} \leq (\zeta_{i^*,1}/(20\anticoncgap)) \cdot \E[\bs_{i^*,1}]  = \ul{\st}_{i^*+1,1}/(20\anticoncgap)
    \]
    except with probability at most
    \[
        \parens*{\frac{4\max\{\sqrt{\zeta_{i^*,1}},\zeta_{i^*,1}\}}{\zeta_{i^*,1}/(2\anticoncgap)}}^\taylor = (8\anticoncgap \max\{\zeta_{i^*,1}^{-1/2},1\})^\taylor.
    \]
    Using again $\zeta_{i^*,1} > 100 \anticoncgap$, this probability bound is at most $(8/10)^\taylor \cdot \anticoncgap^{\taylor/2}$.
\end{proof}

Putting the preceding two claims together, we conclude that
\[
    \bs_{i^*+1,0} \geq 10 \anticoncgap \bs_{i^*,1} \quad \text{except with probability } O(\anticoncgap)^{\taylor/2},
\]
which establishes \Cref{ineq:muffin} for the $i^*$-th strong anticoncentration\rodnote{or local hyperconcentration} mollifier check (using $10 \geq e^2$).

\ignore{
\subsection{If some analysis check fails, then some mollifier check fails with high probability.}  Let's start with an edge case.  I believe the ``bottom row'' ($i = d$) analysis checks cannot actually fail, because not only is each $\ul{s}_{d,j}$ a constant, it should be the \emph{same} constant.  \\

Recall that we consider the analysis checks in this left-to-right, bottom-to-top order.

\paragraph{Case 1: The ``first'' analysis check that fails is a horizontal one.} Say that this first failing check is $\ul{s}_{i^*,j^*} \approxeq \ul{s}_{i^*,j^*+1}$.  Note that $i^* < d$, by virtue of the edge case we took care of, and $j^* < 4d+1$.  Note also that $j^* \geq 1$, with $j^* = 1$ being a bit of a special case.

Let's collect up some things we know by virtue of this $(i^*,j^*)$ being the \emph{first} point of failure.  I'm not sure we'll need \emph{all} the facts we collect up, but why not?  We know:
\begin{itemize}
    \item $\ul{s}_{i^*+1,j} \approxeq \ul{s}_{i^*+1,j+1}$ for all $j > 0$, and hence also for $j = 0$ by the Magic Lemma.  All these values are basically equal to $\ul{s}_{i^*+1,1}$.
    \item $\ul{s}_{i^*,1} \geq \eps^2 \ul{s}_{i^*+1,1}$.  Combining this with the previous bullet point, we get
    \[
       \ul{s}_{i^*,1} \geq \eps^2 \cdot \ul{s}_{i^*+1,j} \quad \forall 0 \leq j \leq 4d+1.
    \]
    \item $\ul{s}_{i^*,1} \approxeq \ul{s}_{i^*,2} \approxeq \cdots \approxeq \ul{s}_{i^*,j^*}$.  Hence combining with the previous bullet point,
    \[
        \ul{s}_{i^*,j'} \geq \eps^2 \cdot \ul{s}_{i^*+1,j} \quad \forall 0 \leq j \leq 4d+1 \quad \forall 1 \leq j' \leq j^*.
    \]
\end{itemize}
Now we're going to study the random variables $\bs_{i^*,j^*-1}$ and $\bs_{i^*,j^*}$.  (Note that $j^*-1$ makes sense, as $j^* \geq 1$.)  We have
\[
    \E[\bs_{i^*,j^*-1}] = \ul{s}_{i^*,j^*}, \qquad \E[\bs_{i^*,j^*}] = \ul{s}_{i^*,j^*+1},
\]
\begin{align*}
    \Var[\bs_{i^*,j^*-1}] &\lesssim p \cdot \ul{s}_{i^*+1,j^*-1} \cdot \ul{s}_{i^*,j^*}  & \Var[\bs_{i^*,j^*}] &\lesssim p \cdot \ul{s}_{i^*+1,j^*} \cdot \ul{s}_{i^*,j^*+1}\\
     &\leq p\eps^{-2} \cdot \ul{s}_{i^*,j^*} \cdot \ul{s}_{i^*,j^*} &  &\leq  p\eps^{-2} \cdot \ul{s}_{i^*,j^*} \cdot \ul{s}_{i^*,j^*+1},
\end{align*}
where the last inequalities used our collected-up facts.  Would look more natural if the last expression had $\ul{s}_{i^*,j^*+1}$ twice, but I guess we aren't eligible to take $j'$ to be that.  But anyway, if we let
\[
    S = \max\{\ul{s}_{i^*,j^*}, \ul{s}_{i^*,j^*+1}\},
\]
we may conclude
\[
    \Var[\bs_{i^*,j^*-1}] \lesssim p \eps^{-2} \cdot S^2, \qquad  \Var[\bs_{i^*,j^*}] \lesssim p \eps^{-2} \cdot S^2;
\]
i.e.,
\[
    \stddev[\bs_{i^*,j^*-1}] \lesssim \eta \cdot S, \qquad  \stddev[\bs_{i^*,j^*}] \lesssim \eta \cdot S,
\]
where I guess I'm really starting to rely on the notation $\eta = \sqrt{p}/\eps$.\\

Okay, so abstracting a bit, we have two random variables $\br_1, \br_2$ with means $\mu_1, \mu_2$.  By the very assumption that the analysis check failed, we have $\mu_1 \not \approxeq \mu_2$.  WLOG say $\mu_2$ is bigger ($S = \mu_2$), so the facts we have are
\[
    \mu_1 \leq (1-(\tfrac{1}{1000})^d) \mu_2, \quad \stddev[\br_1], \stddev[\br_2] \leq \eta \mu_2.
\]
I guess by a Markov/Chebyshev/Hypercontractivity style argument, and tolerating $10000^d$ factors, you can conclude that except with probability at most $2^{O(d)} \eta^4$ ($4$th power if you invoke hypercon), the random variables $\br_1, \br_2$ have a ratio difference of more than $1 \pm (\tfrac{1}{5000})^d)$ or whatever, and therefore fail the associated ``soft mollifier check''.  (Recall that the horizontal mollifier checks only go as far as $j = 4d-1$ vs.\ $j = 4d$, but that's okay.)

\paragraph{Case 2: The ``first'' analysis check that fails is a vertical one.} Say that this first failing check is that
\[
    \ul{s}_{i^*,1} \not \geq \eps^2 \ul{s}_{i^*+1,1} \quad \text{for some $0 \leq i^* < d$.}
\]
Again, let's collect up everything we know given that this was the first point of failure.  Well, remembering to invoke the Magic Lemma, we have
\[
    \ul{s}_{i^*+1,j} \approxeq \ul{s}_{i^*+1,0} \quad \forall 0 \leq j \leq 4d+1; \text{ particularly, for $j = 1$}.
\]
And we also have
\[
    \ul{s}_{i^*+1,1}  \geq \eps^2 \ul{s}_{i^*+2,1}
\]
and
\[
    \ul{s}_{i^*+2,j} \approxeq \ul{s}_{i^*+2,0} \quad \forall 0 \leq j \leq 4d+1; \text{ particularly, for $j = 1$},
\]
provided $i^*+2$ ``exists'' (i.e., provided $i^* \neq d-1$).  We're again going to study two particular random variables: $\br_0 = \bs_{i^*,0}$ and $\br_{1} = \bs_{i^*+1,0}$; using the discussion prior to \Cref{fig:meanvar} we get
\[
    \E[\br_0] = \ul{s}_{i^*,1} \not \geq \eps^2  \ul{s}_{i^*+1,1} = \eps^2 \E[\br_1],
\]
and
\begin{align*}
    \Var[\br_0] &\lesssim p \cdot \ul{s}_{i^*+1,0} \cdot \ul{s}_{i^*,1} &  \Var[\br_1] &\lesssim p \cdot  \ul{s}_{i^*+2,0} \cdot \ul{s}_{i^*+1,1} \\
    & \leq p \eps^{2} \cdot \ul{s}_{i^*+1,1}^2 \text{ (sic, re $\eps^{+2}$)}& & \leq p \cdot \eps^{-2} \cdot \ul{s}_{i^*+1,1}^2.
\end{align*}
(Note that when $i^*+2$ doesn't make sense because $i^* = d-1$, the random variable $\br_1$ is $\bs_{d,0}$ which is constant and therefore has variance~$0$.  So in this case, we have the awesomest upper bound we could hope for on $\Var[\br_1]$ anyway.  So it's okay.)

This is getting so finicky, but okay.  If you study $\br_1$, you see that by the usual Markovy argument, $\br_1$ will be within a constant factor of its mean, call that $\mu_1$, except with probability $O(\eta^4)$.  As for $\br_0$, we know that \emph{its} mean (call it $\mu_0$) is smaller than $\eps^2 \mu_1$, and it's fairly well concentrated around its mean; we have $\stddev[\br_0] \lesssim \eta \eps^2 \mu_1$. So I think again we're exactly in shape to conclude that except with probability at most $O(\eta^4)$, $\br_0 \leq \eps^2 \br_1$ and so the soft mollifier check $\bs_{i^*,0} \geq \eps^2 \bs_{i^*+1,0}$ fails.
}

==> noise-insens-statistics-safe.tex <==
%!TEX root = the-good-life3.tex

\section{Noise insensitivity of the statistics: Proof of \Cref{thm:noise-insensitivity}} \label{sec:noise-insensitivity}

\begin{remark} \label{rem:our-noise-insensitivity-of-statistics-versus-kanes}
Before entering into the proof, we note that \Cref{thm:noise-insensitivity} is analogous to Lemma~11 of \cite{kane11focs}, which shows that for every $i,j,$ for most $\bx \sim \normal(0,1)^n$, the $(i,j)$-th statistic at $\bx$ is multiplicatively close to the $(i,j+1)$-th statistic at $\bx$.  As in \Cref{rem:our-strong-anticoncentration-versus-kanes}, \cite{kane11focs}'s proof of Lemma~11 uses Lemma~9 of that paper, but at this point too the argument of \cite{kane11focs} incurs a $2^d$ factor because of hypercontractivity (essentially the $9^{-d}$ factor in Corollary~4 of \cite{kane11focs} mentioned below), so \cite{kane11focs}'s Lemma~11 has a $2^{O(d)}$ factor in its failure probability.  

Our arguments in this section also use Lemma~9 of \cite{kane11focs}, but they additionally use our Local Hyperconcentration Theorem  and a quantitative strengthening of Corollary~4 of \cite{kane11focs} for attenuated polynomials which we state and prove below. These latter two new ingredients let us avoid the $2^{O(d)}$ factor which is incurred at this point in the \cite{kane11focs} argument.
\end{remark}

\subsection{Attenuated polynomials are strongly concentrated}

The following lemma\ignore{, which we will use in the proof of \Cref{thm:noise-insensitivity},} says that any attenuated polynomial is strongly concentrated.  This may be viewed as a significant quantitative strengthening of Corollary~4 of \cite{kane11focs}, which states that for any degree-$d$ polynomial $g$, we have $\Prx_{\bx \sim \normal(0,1)^n}[|g(\bx)|\geq \|g\|_2/2] \geq 9^{-d}/2$; in words, $g$ is at least slightly likely to have magnitude at least half of its 2-norm.  In contrast, for attenuated polynomials \Cref{lem:our-cor4} states that with very high probability the magnitude is multiplicatively very close to the 2-norm.

\begin{lemma} [Strong concentration for attenuated polynomials\ignore{; our version of \cite{kane11focs}'s Corollary~4}] \label{lem:our-cor4} Let $0 < \eps,\tau,\delta_1 < 1$ satisfy $ \eps \leq {\frac 1 {(2e \ln(d/\tau))^3}}$ and let $q$ be an $(\hypergeneric,\eps)$-attenuated polynomial of degree at most $d$, where \rasnote{Constraint on $\hypergeneric$} $\hypergeneric \geq \max\{{\frac {4 \eps^{1/3}} {\delta_1}},$ $2ed \ln {\frac d \tau}\}.$   Then
\[
\Prx_{\bx \sim \normal(0,1)^n}\bracks*{|q(\bx)| \approx_{\delta_1} \|q\|_2} \geq 1-\tau.
\]
%\[\Prx_{\bx \sim \normal(0,1)^n}\bracks*{|q(\bx)| \in \red{\left(1 \pm {\frac 1 {\poly(d)}}\right)}\|q\|_2} \geq \red{1-{\frac 1 {\exp(\poly(d))}}}.\]
\end{lemma}

\begin{proof}
Since $q$ is $(\hypergeneric,\eps)$-attenuated, as an immediate consequence of \Cref{def:attenuated} we have that
for each $j=1,\dots,\degree$, 
\begin{equation} \label{eq:apple}
\|q^{=j}\|_2  \leq {\frac {\sqrt{\eps}}{\hypergeneric^{j}}} \cdot \|q\|_2.
\end{equation}

Decomposing $q$ into a sum of orthogonal components $q = q^{=0} + \cdots + q^{=\degree}$, by the triangle inequality we have that
\begin{equation*}
|q^{=0}|=\|q^{=0}\|_2 \in \bracks*{
\|q\|_2 - \sum_{j=1}^\degree \|q^{=j}\|_2, \|q\|_2 + \sum_{j=1}^\degree \|q^{=j}\|_2
},
\end{equation*}
which together with \Cref{eq:apple} immediately yields
\begin{equation} \label{eq:triangle}
|q^{=0}| \approx_{{\frac {2 \sqrt{\eps}}{\hypergeneric}}} \|q\|_2.
\end{equation}

Fix any $j \in \{1,\dots,\degree\}.$ We will apply the tail bound \Cref{thm:tail-bound} to the degree-$j$ polynomial $q^{=j}$, with the ``$t$'' parameter of \Cref{thm:tail-bound} set to\ignore{\rasnote{This is kind of annoying, to have to have a separate definition in the $j=1$ case.  It's because we want something like
$t_j {\frac {\sqrt{\eps}}{\hypergeneric^j}} \leq {\frac {\sqrt{\eps}}{d \hypergeneric}}$ to hold, but since $t_j$ has to be slightly largish (surely at least 1), this doesn't fly when $j=1$ because you don't get the power-of-$\hypergeneric$ helping you in the denominator.  So as a hack we settle for $t_1 {\frac {\sqrt{\eps}}{\hypergeneric^1}} \leq {\frac {\eps^{1/3}}{\hypergeneric}}$ instead. Hacky, sorry. But none of this matters I think.}}
\[
t_j := 
\begin{cases}
{\frac 1 {\eps^{1/6}}} & \text{~if~}j=1;\\
{\frac {\hypergeneric^{j-1}}d} & \text{if~}j \in \{2,\dots,\degree\}.
\end{cases}
\]
The condition on $\eps$ ensures that $t_1 \geq \parens*{{\frac {2e}{j} \ln {\frac \degree \tau}}}^{j/2} \geq \sqrt{2e}$, and the condition on $\hypergeneric$ ensures that for $j=2,\dots,\degree$ we have $t_j \geq \max\{\sqrt{2e}^j,({\frac {2e} j} \ln {\frac d \tau})^{j/2}\}$. So we may apply \Cref{thm:tail-bound}, and we get that for each $j \in \{1,\dots,d\}$,
\begin{equation} \label{eq:first-cb}
\Pr_{\bx \sim \normal(0,1)^n}\bracks*{|q^{=j}(\bx)| > t_j\|q^{=j}\|_2} \leq \exp\left(-\frac{j}{2e}t_j^{2/j} \right)
\leq {\frac \tau \degree}.
\end{equation}
Combining this with \Cref{eq:apple}, we get that

\begin{equation} \label{eq:second-cb}
\Pr_{\bx \sim \normal(0,1)^n}\bracks*{|q^{=j}(\bx)| > t_j \cdot {\frac {\sqrt{\eps}}{\hypergeneric^{j}}} \cdot \|q\|_2} 
\leq {\frac \tau \degree}.
\end{equation}

Now, if $j=1$ we have that $t_1 {\frac {\sqrt{\eps}}{\hypergeneric}} = {\frac {\eps^{1/3}}{\hypergeneric}}$, and if $j \in \{2,\dots,\degree\}$ we have that
$t_j {\frac {\sqrt{\eps}}{\hypergeneric^j}} = {\frac {\sqrt{\eps}}{d \hypergeneric}}$. So by a union bound over all $j=1,\dots,\degree$ and the triangle inequality, we have that with probability at least $1-\tau$ over $\bx \sim \normal(0,1)^n$,
\begin{equation} \label{eq:abra}
\abs*{\sum_{j=1}^\degree q^{=j}(\bx)}
\leq 
\sum_{j=1}^\degree \abs*{q^{=j}(\bx)}  \leq {\frac {\sqrt{\eps} + \eps^{1/3}}{\hypergeneric}} \|q\|_2.
\end{equation}
Since  
\[
|q^{=0}| - \sum_{j=1}^\degree\abs*{q^{=j}(x)} 
\leq 
|q(\bx)| 
\leq
|q^{=0}| + \sum_{j=1}^\degree\abs*{q^{=j}(x)}
\]
holds for all $x$, combining \Cref{eq:triangle} and \Cref{eq:abra} we get that
\[
|q(\bx)| \approx_{{\frac {4 \eps^{1/3}}{\hypergeneric}}} \|q\|_2,
\]
\ignore{
%\[\|q^{=0}\| \in \bracks*{\parens*{1 - {\frac {4 \eps^{1/3}}{\hypergeneric}}} \|q\|,\parens*{1 + {\frac {4 \eps^{1/3}}{\hypergeneric}}} \|q\|}\]
}
which gives the lemma by the condition on $\hypergeneric$ in the lemma statement.
\end{proof}

%Similar to the previous section, what we actually need is a generalized version of the above statement, which applies to a family of polynomials.  This is the following:

%\begin{lemma} [Strong concentration for an attenuated-on-average family of polynomials] \label{lem:our-cor4} Let $(p_\upsilon)_{\upsilon \in \Upsilon}$ be a family of polynomials of degree at most $d$ that is $\hypergeneric$-attenuated on average, where $\hypergeneric \geq \red{fill-in(\tau,\delta_1)}.$   Then \blue{(FINISH THIS)}
%\[
%\Prx_{\bx \sim \normal(0,1)^n}\bracks*{|q(\bx)| \in \red{\left(1 \pm \delta_1\right)}\|q\|_2} \geq 1-\tau.
%\]
%\[\Prx_{\bx \sim \normal(0,1)^n}\bracks*{|q(\bx)| \in \red{\left(1 \pm {\frac 1 {\poly(d)}}\right)}\|q\|_2} \geq \red{1-{\frac 1 {\exp(\poly(d))}}}.\]
%\end{lemma}


\ignore{
%\gray{
%\noindent {\emph{Proof sketch:}}
%\ignore{\footnote{We could have $\hat{q}(0)$ in place of $\|q\|_2$ above. if we wanted.}} The argument giving this uses a degree-$k$ Chernoff bound for the level-$k$ portion, for every $1 \leq k \leq d$; thanks to the attenuation, such a degree-$k$  Chernoff bound will give that for each $k$, the displacement of $q^{=k}(\bx)$ away from $\hat{q}(0)$ is at most $\|q\|_2/\poly(d)$ except with $1/\exp(\poly(d))$ failure probability. Then a union bound gives the statement.  

%\blue{What we need to do here is highly reminiscent of what's done in the proof of \Cref{lem:HZL-2-norm-retention}, consult that.}}
%
}


%\rasnote{Note that while we have an inverse exponential failure probability above, if we are starting with an arbitrary polynomial $p$ and we get $q$ via the RZL as $q(y)=p_{\lambda | x}(y)$ (now we're calling the argument $y$), then the probability that $q$ is strongly attenuated in the first place will only be $1 - 1/\poly(d).$}

\subsection{The main technical lemma for \Cref{thm:noise-insensitivity}}
As we explain in the next subsection, \Cref{thm:noise-insensitivity} follows rather directly from \Cref{lem:our-lem11}, which is the main result of this subsection.  The proof requires the following anticoncentration result from \cite{kane11focs}, which intuitively says that the value of a polynomial is likely to be very stable, in a multiplicative sense, when moving from a random point to a random zoom centered at that random point.

\begin{lemma} [Anticoncentration for degree-$\degree$ polynomials; Lemma~9 of \cite{kane11focs}] \label{lem:kane-lemma9}
Let $g$ be any degree-$\degree$ polynomial over Gaussian space.  Suppose that $0 < \noisegeneric < \kappa/100$.  Then with probability at least $1-O(d^2 \kappa)$ over independent $\bx,\by \sim \normal(0,1)^n$, it holds that
\[
|\zoom{g}{\noisegeneric}{\bx}(\by)| \approx_{{\frac \noisegeneric \kappa}} |g(\bx)|.
\]
\end{lemma}

\begin{lemma} [Variant of Daniel's Lemma~11, ``large-$\lambda$ regime'']\label{lem:our-lem11} 
Let $(g_\bup)_{\bupsilon \sim \Upsilon}$ be a nice (in the sense of \Cref{sec:distributional}) distribution of polynomials over $\R^n$ of degree at most $\degree$.
Let $\noisegeneric' := \blue{BLAH1(\degree,\rho,\mu)}$, and suppose that $0 < \rho < {\frac 1 {100}}$, $\noisegeneric' \leq \blue{BLAH2(\degree,\rho,\mu)}$.  Then with probability at least $1-\mu$ over $\bx \sim \normal(0,1)^n$, we have that
\[
\Ex_{\by \sim \normal(0,1)^n}
\bracks*{\Ex_{\bup}\bracks*{
\zoom{(g_{\bup})}{\noisegeneric'}{\bx}(\by)^2}}
\approx_\rho
\Ex_{\bup}\bracks*{g_{\bup}(\bx)^2}.
\]
\end{lemma}

\begin{proof}
For $x \in \R^n$, we define the quantities
\begin{align}
C_x&:= \Ex_{\bup}\bracks*{g_{\bup}(x)^2}, \label{eq:Cdef}\\
r_x(y) &:= \Ex_{\bup}\bracks*{\zoom{(g_{\bup})}{\noisegeneric'}{x}(y)^2},  \text{~and~}\label{eq:rxydef}\\
q_x(y) &:= r(x,y) - C(x). \label{eq:qxy}
\end{align}
As suggested by the notation, given a fixed $x \in \R^n$, the quantity $C_x$ should be thought of as a ``constant,'' whereas $r_x(y)$ and $q_x(y)$ are polynomials in $y$ of degree at most $2d$.

For notational convenience, for $x \in \R^n$ we define the shorthand 
\[
\text{``$A(x)$'' to mean the event ``}\Ex_{\by} \bracks*{\Ex_{\bup}\bracks*{\zoom{(g_{\bup})}{\noisegeneric'}{x}(\by)^2}} \not\approx_{\rho} \Ex_{\bup}\bracks*{g_{\bup}(\bx)^2}\text{,'' i.e., ``}
\Ex_{\by}[r_x(\by)] \not \approx_\rho C_x\text{,''}
\]
and the goal of the proof is to show that $p_A \leq \mu$, where $p_A := \Pr_{\bx}[A(\bx)].$



Our argument below will use the following simple fact:

\begin{fact} \label{fact:rx-attenuated} Let $\noisegeneric',\beta,\kappa,\hypergeneric$ be such that \rasnote{This condition was ``$
            \hypergeneric  \ge  \frac{C d \log d \cdot \sqrt{\log(1/\beta)}}{\beta},
$'', the new condition is propagated from \Cref{thm:HZL}}
\begin{equation}
  \noisegeneric' \leq \kappa \cdot \parens*{\frac{ \beta}{d \hypergeneric}}^{C \log d},
\quad \quad 
   \blue{ \hypergeneric  \ge  \frac{C \degree \log \degree \cdot \sqrt{\log \log \degree + \log(1/\beta)}}{\beta}}
   \label{eq:rxattenuated}
\end{equation}
where $C$ is a suitably large absolute constant. Then with probability at least $1-\beta$ over $\bx \sim \normal(0,1)^n$, the polynomial $r_\bx(y)$ is $(\hypergeneric,\kappa)$-attenuated.
\end{fact}

\begin{proof}
This is a direct consequence of \Cref{thm:RZL}, our random zoom lemma for a single polynomial.  Define  
\[
P(y) := \Ex_{\bup}[g_{\bup}(y)^2],
\] 
and observe that $P(y)$ is a polynomial of degree at most $2d$. Applying \Cref{thm:RZL} to $P$, we get that except with probability at most $\beta$ the polynomial $\zoom{P}{\noisegeneric'}{\bx}$ is $(\hypergeneric,\kappa)$-attenuated, and the fact follows since
\[
\zoom{P}{\noisegeneric'}{\bx}(y)
=
P(\sqrt{1-\noisegeneric'} \bx + \sqrt{\noisegeneric'} y)\\
=
\Ex_{\bup}[g_{\bup}(\sqrt{1-\noisegeneric'} \bx + \sqrt{\noisegeneric'} y)^2]\\
=
\Ex_{\bup}[\zoom{(g_{\bup})}{\noisegeneric'}{\bx}(y)^2]\\
= r_{\bx}(y). \qedhere
\]
\end{proof}

We will also use the following:

\begin{claim} \label{claim:r-to-q}
For $\kappa < 1/10$, if $x$ is such that both (i) $r_x(y)$ is $(\hypergeneric,\kappa)$-attenuated and (ii) $A(x)$ holds, then $q_x(y)$ is $(\hypergeneric,8\kappa/\rho^2)$-attenuated.
\end{claim}

We defer the proof of \Cref{claim:r-to-q} until \Cref{sec:r-to-q} and continue with the proof of \Cref{lem:our-lem11}. Towards the goal of upper bounding $p_A$, we first observe that by \Cref{fact:rx-attenuated}, taking its ``$\hypergeneric$'' parameter to be $\hyperfixed$, its ``$\kappa$'' parameter to be $c \rho^2 / (\log \degree)^3$ for a suitably small constant $c$, its $\noisegeneric'$ parameter to be \blue{AAA} and its $\beta$ parameter to be $\mu/2$, and observing that these parameter settings satisfy \Cref{eq:rxattenuated}, \red{tricky:  $\mu$ won't be set until \Cref{sec:proof-of-thm-noise-insens-using-our-lem-11}} we have that
\[
\Pr_{\bx}[A(\bx) \text{~holds and~}r_{\bx}(y) \text{~is~}(\hypergeneric,\kappa)\text{-attenuated}]
\geq p_A - \mu/2,
\]
and from this, by \Cref{claim:r-to-q}, we get that
\begin{equation} \label{eq:goodie}
\Pr_{\bx}[A(\bx) \text{~holds and~}q_{\bx}(y) \text{~is~}(\hypergeneric,8\kappa/\rho^2)\text{-attenuated}]
\geq p_A - \mu/2.
\end{equation}
In the rest of the argument we will upper bound the probability on the left-hand side of \Cref{eq:goodie} and thereby upper bound $p_A$.

So, let us fix an outcome $x$ satisfying the condition of \Cref{eq:goodie}, i.e. an $x$ such that $A(x)$ holds and $q_{x}(y)$ is $(\hypergeneric,8\kappa/\rho^2)$-attenuated.
We apply \Cref{lem:our-cor4} to the polynomial $q_x$, taking the ``$\delta_1$'' and ``$\tau$'' parameters in \Cref{lem:our-cor4} to each be $1/2$, taking its ``$\eps$'' parameter to be $8\kappa/\rho^2$, and taking its ``$\hypergeneric$'' parameter to be $\hyperfixed$. (It is straightforward to verify that for these settings, the $\hypergeneric$ and $\eps$ of \Cref{lem:our-cor4} indeed satisfy the bounds required in that lemma statement.)
Since $A(x)$ holds we have $|\Ex_{\by}[q_x(\by)]| \geq \rho \Ex_{\bup}[g_\bup(x)^2]$, and since $\|q_x\| \geq |\wh{q_x}(0^n)| = |\Ex_{\by}[q_x(\by)]|,$ it follows that 
$\|q_x\| \geq \rho \Ex_{\bup}[g_\bup(x)^2]$, so we get from \Cref{lem:our-cor4} that
\[
|q_x(\by)| =
|\Ex_{\bup}\bracks*{\zoom{(g_\bup)}{\noisegeneric'}{x}(\by)^2} - \Ex_{\bup}\bracks*{g_\bup(x)^2}|
\geq  \|q_x\|/2 \geq (\rho/2)\Ex_{\bup}[g_\bup(x)^2] 
\]
with probability at least $1/2$ over $\by$. 

For $x,y \in \R^n$ let us define the shorthand
\[
\text{``$B(x,y)$'' to mean the event ``}\Ex_{\bup}\bracks*{\zoom{(g_\bup)}{\noisegeneric'}{x}(y)^2} \not\approx_{\rho/2} \Ex_{\bup}\bracks*{g_\bup(x)^2}\text{,'' i.e. ``}
r_x(\by)] \not\approx_{\rho/2} C_x\text{.''}
\]
Summarizing the preceding paragraph, it showed that if $x$ is such that $A(x)$ holds and $q_x$ is $(\hypergeneric,8\kappa/\rho^2)$-attenuated, then with probability at least 
$1/2$ over $\by$, we have that $B(x,\by)$ holds.

Now we apply \Cref{lem:kane-lemma9} to get an upper bound on $\Pr[B(\bx,\by)]$, with its ``$\noisegeneric$'' parameter set to $\noisegeneric'$ and its ``$\kappa$'' parameter set to $2 \noisegeneric'/\rho$ (so the ``$\noisegeneric/\kappa$'' of \Cref{lem:kane-lemma9} is $\rho/2$), and its polynomial ``$p$'' being $\Ex_{\bup}[g_\bup^2].$  Applied in this way we see that \Cref{lem:kane-lemma9} gives $\Pr[B(\bx,\by)] \leq O(d^2 \kappa) = O(d^2 \noisegeneric'/\rho)$. 
Combining this with the last sentence of the previous paragraph, it must hold that
\begin{equation} \label{eq:gumdrops}
 \Pr_{\bx}[A(\bx) \text{~holds and~}q_{\bx}\text{~is $(\hypergeneric,8\kappa/\rho^2)$-attenuated}] \leq  2 \cdot O(d^2 \noisegeneric'/\rho) =
O(d^2) \cdot \noisegeneric'/\rho.
 \end{equation}
Combining \Cref{eq:goodie} and \Cref{eq:gumdrops}, we get that $p_A \leq O(d^2) \cdot \noisegeneric'/\rho + \mu/2$. Recalling the setting of $\noisegeneric' = \blue{AAA}$ we have that the right-hand side of \Cref{eq:gumdrops} is at most $\mu$, and \blue{Verify $O(d^2) \cdot \noisegeneric'/\rho \leq \mu/2$]]]} \Cref{lem:our-lem11} is proved.
\end{proof}

\subsubsection{Proof of \Cref{claim:r-to-q}} \label{sec:r-to-q}

Recall that by the assumption of the claim, we have that $r_x$ is $(\hypergeneric,\kappa)$-attenuated and that $A(x)$ holds.  The latter can be rephrased as
\[
\E[r_x(\by)] \not\approx_{\rho} C_x.
\]
Recalling that $q_x(y)=r_x(y)-C_x,$ it follows that $\wh{q_x}(0^n) = \E[q_x(\by)] \notin [-\rho C_x, \rho C_x].$
Now we consider two possibilities.  First, if $0 \leq \E[r_x(\by)] \leq (1-\rho)C_x$, then since $C_x \geq {\frac {\E[r_x(\by)]}{1-\rho}}$ we have 
\[
|\wh{q_x}(0^n)| \geq \rho C_x \geq {\frac \rho {1-\rho}} \E[r_x(\by)] \geq \rho |\wh{r_x}(0^n)|
\]
(where we used the nonnegativity of $r_x$ for the last inequality).
Second, if $(1+\rho)C_x \leq \E[r_x(\by)]$, then since $-C_x \geq {\frac {-\E[r_x(\by)]}{1+\rho}}$ we have
\[
\wh{q_x}(0^n)=\E[q_x(\by)] = \E[r_x(\by)] - C_x \geq \E[r_x(\by)] \left( 1 -  {\frac 1 {1+\rho}}\right) \geq (\rho/2) \E[r_x(\by)] = (\rho/2)|\wh{r_x}(0^n)|
\]
(where the second inequality uses $0 < \rho < 1/100$). So in both cases we have $|\wh{q_x}(0^n)| \geq (\rho/2)|\wh{r_x}(0^n)|$, and hence we have that
\begin{equation} \label{eq:qxemptysetnottoosmall}
|\wh{q_x}(0^n)|  \geq (\rho/2) |\wh{r_x}(0^n)|
\end{equation}
In words, this says that  the constant Hermite coefficient of $q_x$ is (multiplicatively) smaller than the constant Hermite coefficient of $r_x$ by at most a  $\rho/2$ multiplicative factor. 

To finish the proof, we observe that since the polynomial $r_x$ is $(\hypergeneric,\kappa)$-attenuated where $\kappa \leq 1/10$, it must be the case that the magnitude of the constant Hermite coefficient $|\wh{r_x}(0^n)|$ contributes the lion's share of  $\|r_x\|$ --- to be more precise, it must hold that
$\wh{r_x}(0^n)^2 \geq \|r_x\|^2/2.$  Since $\HV_\hypergeneric[q_x^{>0}]=\HV_\hypergeneric[r_x^{>0}]$ (since $q_x$ and $r_x$ differ only in the constant term $C_x$), and $\|q_x\| \geq |\wh{q_x}(0^n)|$, recalling \Cref{eq:qxemptysetnottoosmall} we can infer from $r_x$ being $(\hypergeneric,\kappa)$-attenuated that $q_x$ is $(\hypergeneric,8\kappa/\rho^2)$-attenuated.
This proves \Cref{claim:r-to-q}. \qed







\subsection{Proof of \Cref{thm:noise-insensitivity} using \Cref{lem:our-lem11}} \label{sec:proof-of-thm-noise-insens-using-our-lem-11}

Fix an $i \in \{0,\dots,\degree\}$ and a $j \in \{0,\maxcol-1\}$. We apply \Cref{lem:our-lem11} taking the nice distribution $(g_\bup)_{\bup \sim \Upsilon}$ to be ${\cal F}_{i,j}$, taking its parameter ``$\noisegeneric'$'' to be
$\noisefixed$, taking its parameter ``$\rho$'' to be $\horizclose$, and taking its parameter ``$\mu$'' to be $\epsprg/(8(\degree+1)\maxcol)$. Recalling the setting of $\noisefixed$ from \Cref{eq:noisefixed}, we \blue{[[[Confirm that condition $\noisegeneric' \leq \blue{BLAH}$ is satisfied]]]}.   By \Cref{eq:alt-sij} we have that $\st_{i,j}(x)=\Ex_{\bup}[g_{\bup}(x)^2]$, and by \Cref{eq:stats-as-zooms} we have that
\[
\Ex_{\by \sim \normal(0,1)^n}
\bracks*{\Ex_{\bup}\bracks*{
\zoom{(g_{\bup})}{\noisegeneric'}{x}(\by)^2}}=
\Ex_{\bup}
\bracks*{\Ex_{\by}\bracks*{
\zoom{(g_{\bup})}{\noisegeneric'}{x}(\by)^2}} =
\Ex_{\bup}
\bracks*{\norm*{\zoom{(g_{\bup})}{\noisegeneric'}{x}}_2^2
}=\st_{i,j+1}(x).
\]
So \Cref{lem:our-lem11} gives that except with probability at most $\epsprg/(8(\degree+1)\maxcol)$ over $\bx \sim \normal(0,1)^n,$ we have
\[
\st_{i,j}(\bx) \approx_{\horizclose} \st_{i,j+1}(\bx),
\]
and \Cref{thm:noise-insensitivity} is proved. \qed



